On the Computation Power of Name Parameterization in Higher-order Processes

Parameterization extends higher-order processes with the capability of abstraction (akin to that in lambda-calculus), and is known to be able to enhance the expressiveness. This paper focuses on the parameterization of names, i.e. a construct that maps a name to a process, in the higher-order setting. We provide two results concerning its computation capacity. First, name parameterization brings up a complete model, in the sense that it can express an elementary interactive model with built-in recursive functions. Second, we compare name parameterization with the well-known pi-calculus, and provide two encodings between them.

==> eptcsdata.tex <==
\providecommand{\firstpage}{114}
\providecommand{\publicationstatus}{S. Knight, I. Lanese, A. Lluch Lafuente and H. T. Vieira (Eds.):\\ 8th Interaction and Concurrency Experience (ICE 2015)\\
EPTCS 189, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.189.10}{10.4204/EPTCS.189.10}}
\pdfoutput=1

